HDSDP: Software for Semidefinite Programming

HDSDP is a numerical software solving the semidefinite programming problems. The main framework of HDSDP resembles the dual-scaling interior point solver DSDP [BY2008] and several new features, including a dual method based on the simplified homogeneous self-dual embedding, have been implemented. The embedding technique enhances stability of the dual method and several new heuristics and computational techniques are designed to accelerate its convergence. HDSDP aims to show how dual-scaling algorithm benefits from the self-dual embedding and it is developed in parallel to DSDP5.8. Numerical experiments over several classical benchmark datasets exhibit its robustness and efficiency, and particularly its advantages on SDP instances featuring low-rank structure and sparsity. HDSDP is open-sourced under MIT license and available at https://github.com/COPT-Public/HDSDP.

==> diag-clean.tex <==
This section presents the detailed solution statistics of \texttt{HDSDP} on diagonal pre-conditioning problems.
If an instance fails, its solution time is recorded as 3600 seconds.

\subsection{Summary Statistics}

\begin{table}[H]
\caption{Summary statistics on diagonal pre-conditioning problems}
  \begin{tabular}{ccc}
  \toprule
  Solver & Number of solved instances & Shifted geometric mean \\
  \midrule
  \texttt{HDSDP} & 6 & 34.78 \\
    \texttt{DSDP5.8} & 4 & 396.85 \\
    \texttt{COPT v6.5} & 5 & 148.39 \\
  	\bottomrule
  \end{tabular}	
\end{table}

\subsection{Detailed Solution Statistic}

{\small{\begin{table}[H]
  \begin{center}
    \caption{Diagonal pre-conditioning problems with \texttt{HDSDP}}
  \resizebox{0.8\textwidth}{!}{%
  \begin{tabular}{cccccccr}
      \toprule
      Instance & Error 1 & Error 2 & Error 3 & Error 4 & Error 5 & Error 6 &
      Time\\
\midrule
diag-bench-1000-1.000e-02-L & 3.58e-13 & 0.00e+00 & 5.41e-10 & 0.00e+00 & 2.12e-07 & 2.85e-07 & 37.670 \\ 
diag-bench-2000-5.000e-02-L & 1.23e-13 & 0.00e+00 & 1.83e-10 & 0.00e+00 & 6.39e-07 & 7.48e-07 & 276.960 \\ 
             diag-bench-DK01R-L & 2.08e-14 & 0.00e+00 & 0.00e+00 & -0.00e+00 & 2.87e-03 & 2.87e-03 & 5.010 \\ 
    diag-bench-micromass\_10NN-L & 6.32e-15 & 0.00e+00 & 6.11e-10 & 0.00e+00 & 3.98e-07 & 4.53e-07 & 20.510 \\ 
          diag-bench-west0989-L & 1.11e-15 & 0.00e+00 & 3.01e-07 & 0.00e+00 & -4.54e-04 & 2.00e-03 & 35.280 \\ 
      \bottomrule
    \end{tabular}
}  
\end{center}
\end{table}}}


{\small{\begin{table}[H]
  \begin{center}
    \caption{Diagonal pre-conditioning problems with \texttt{DSDP5.8}}
  \resizebox{0.8\textwidth}{!}{%
  \begin{tabular}{cccccccr}
      \toprule
      Instance & Error 1 & Error 2 & Error 3 & Error 4 & Error 5 & Error 6 &
      Time\\
\midrule
diag-bench-1000-1.000e-02-L & 1.48e-11 & 0.00e+00 & 0.00e+00 & 0.00e+00 & 3.52e-07 & 3.53e-07 & 207.500 \\ 
diag-bench-2000-5.000e-02-L & 6.51e-13 & 0.00e+00 & 0.00e+00 & 0.00e+00 & 1.91e-07 & 1.92e-07 & 971.700 \\ 
             diag-bench-DK01R-L & 1.85e+02 & 0.00e+00 & 0.00e+00 & 0.00e+00 & 9.97e-01 & 1.58e+00 & Failed \\ 
    diag-bench-micromass\_10NN-L & 5.98e-11 & 0.00e+00 & 0.00e+00 & 0.00e+00 & 4.46e-07 & 4.51e-07 & 38.450 \\ 
          diag-bench-west0989-L & 8.11e-01 & 0.00e+00 & 0.00e+00 & 0.00e+00 & 6.77e-01 & 7.07e-01 & Failed \\ 
      \bottomrule
    \end{tabular}
}  
\end{center}
\end{table}}}


{\small{\begin{table}[H]
  \begin{center}
    \caption{Diagonal pre-conditioning problems with \texttt{COPT}}
  \resizebox{0.8\textwidth}{!}{%
  \begin{tabular}{cccccccr}
      \toprule
      Instance & Error 1 & Error 2 & Error 3 & Error 4 & Error 5 & Error 6 &
      Time\\
\midrule
diag-bench-1000-1.000e-02-L & 3.72e-13 & 0.00e+00 & 0.00e+00 & 0.00e+00 & 1.55e-07 & 7.02e-06 & 38.610 \\ 
diag-bench-2000-5.000e-02-L & 5.67e-13 & 0.00e+00 & 0.00e+00 & 0.00e+00 & 2.47e-08 & 1.64e-06 & 161.170 \\ 
             diag-bench-DK01R-L & 3.53e-05 & 0.00e+00 & 0.00e+00 & 0.00e+00 & 1.78e-02 & 2.35e-03 & Failed \\ 
    diag-bench-micromass\_10NN-L & 4.30e-10 & 0.00e+00 & 0.00e+00 & 0.00e+00 & 5.21e-10 & 7.09e-10 & 17.430 \\ 
          diag-bench-west0989-L & 2.41e-08 & 0.00e+00 & 0.00e+00 & 0.00e+00 & 1.21e-05 & 1.83e-06 & 76.900 \\ 

      \bottomrule
    \end{tabular}
}  
\end{center}
\end{table}}}



==> sdplib-clean.tex <==
This section summarizes the benchmark result of \texttt{HDSDP} on \texttt{SDPLIB} \cite{borchers1999sdplib}. The main setup is consistent with the experiment section. If an instance fails, its solution time is recorded to be 3600 seconds.

\subsection{Summary Statistics}

\begin{table}[H]
\caption{Summary statistics on \texttt{SDPLIB} benchmark}
  \begin{tabular}{ccc}
  \toprule
  Solver & Number of solved instances & Shifted geometric mean \\
  \midrule
  \texttt{HDSDP} & 91 & 3.58 \\
    \texttt{DSDP5.8} & 89 & 4.51 \\
    \texttt{COPT v6.5} & 92 & 3.43 \\
  	\bottomrule
  \end{tabular}	
\end{table}

\subsection{Detailed Solution Statistic}
\begin{table}[H]
\caption{Tables of detailed solution statistics}
  \begin{tabular}{cc}
  \toprule
  Solver & Table \\
  \midrule
   \texttt{HDSDP} & Table \ref{sdplib-hdsdp-1} and  \ref{sdplib-hdsdp-2}   \\
    \texttt{DSDP5.8} & Table \ref{sdplib-dsdp-1} and  \ref{sdplib-dsdp-2} \\
    \texttt{COPT v6.5} & Table \ref{sdplib-copt-1} and  \ref{sdplib-copt-2} \\
  	\bottomrule
  \end{tabular}	
\end{table}
{\small{\begin{table}[h]
  \begin{center}
    \caption{SDPLIB benchmark \texttt{HDSDP}, Part 1} \label{sdplib-hdsdp-1}
  \resizebox{0.75\textwidth}{!}{%
  \begin{tabular}{cccccccc}
      \toprule
      Instance & Error 1 & Error 2 & Error 3 & Error 4 & Error 5 & Error 6 &
      Time\\
\midrule
               arch0 & 8.82e-13 & 0.00e+00 & 0.00e+00 & -0.00e+00 & 4.03e-07 & 2.21e-07 & 0.350 \\ 
               arch2 & 1.20e-12 & 0.00e+00 & 0.00e+00 & -0.00e+00 & 2.84e-07 & 1.54e-07 & 0.370 \\ 
               arch4 & 1.37e-13 & 0.00e+00 & 0.00e+00 & -0.00e+00 & 2.57e-07 & 1.39e-07 & 0.360 \\ 
               arch8 & 9.48e-12 & 0.00e+00 & 0.00e+00 & -0.00e+00 & 4.49e-07 & 2.76e-07 & 0.430 \\ 
           control10 & 1.01e-06 & 0.00e+00 & 0.00e+00 & -0.00e+00 & 9.70e-06 & 9.27e-06 & 9.720 \\ 
           control11 & 1.67e-06 & 0.00e+00 & 0.00e+00 & -0.00e+00 & 1.43e-05 & 1.34e-05 & 15.250 \\ 
            control1 & 4.65e-07 & 0.00e+00 & 0.00e+00 & -0.00e+00 & 4.75e-07 & 1.45e-07 & 0.040 \\ 
            control2 & 6.82e-07 & 0.00e+00 & 0.00e+00 & -0.00e+00 & 2.22e-07 & 1.42e-07 & 0.070 \\ 
            control3 & 1.10e-06 & 0.00e+00 & 0.00e+00 & -0.00e+00 & -1.32e-08 & 2.59e-07 & 0.110 \\ 
            control4 & 8.83e-07 & 0.00e+00 & 0.00e+00 & -0.00e+00 & -3.56e-07 & 5.17e-07 & 0.260 \\ 
            control5 & 1.95e-06 & 0.00e+00 & 0.00e+00 & -0.00e+00 & 1.22e-06 & 7.68e-07 & 0.790 \\ 
            control6 & 1.97e-08 & 0.00e+00 & 0.00e+00 & -0.00e+00 & 1.12e-05 & 1.12e-05 & 0.950 \\ 
            control7 & 3.99e-06 & 0.00e+00 & 0.00e+00 & -0.00e+00 & 1.00e-06 & 4.78e-07 & 2.070 \\ 
            control8 & 3.74e-06 & 0.00e+00 & 0.00e+00 & -0.00e+00 & 2.65e-04 & 2.67e-04 & 6.410 \\ 
            control9 & 5.40e-06 & 0.00e+00 & 0.00e+00 & -0.00e+00 & 7.80e-06 & 1.04e-05 & 7.410 \\ 
            equalG11 & 7.45e-14 & 0.00e+00 & 0.00e+00 & -0.00e+00 & 5.34e-07 & 5.34e-07 & 5.810 \\ 
            equalG51 & 1.72e-12 & 0.00e+00 & 0.00e+00 & -0.00e+00 & 2.02e-07 & 2.02e-07 & 12.110 \\ 
              gpp100 & 1.36e-07 & 0.00e+00 & 0.00e+00 & -0.00e+00 & -1.77e-07 & 2.57e-07 & 0.050 \\ 
            gpp124-1 & 2.16e-06 & 0.00e+00 & 0.00e+00 & -0.00e+00 & -4.71e-06 & 2.01e-07 & 0.070 \\ 
            gpp124-2 & 3.70e-08 & 0.00e+00 & 0.00e+00 & -0.00e+00 & 4.97e-07 & 5.84e-07 & 0.060 \\ 
            gpp124-3 & 2.63e-08 & 0.00e+00 & 0.00e+00 & -0.00e+00 & 7.38e-08 & 1.95e-07 & 0.060 \\ 
            gpp124-4 & 1.27e-08 & 0.00e+00 & 0.00e+00 & -0.00e+00 & 3.05e-07 & 2.74e-07 & 0.060 \\ 
            gpp250-1 & 2.46e-06 & 0.00e+00 & 0.00e+00 & -0.00e+00 & -1.05e-05 & 3.35e-07 & 0.200 \\ 
            gpp250-2 & 1.34e-07 & 0.00e+00 & 0.00e+00 & -0.00e+00 & -2.20e-07 & 3.54e-07 & 0.170 \\ 
            gpp250-3 & 2.03e-08 & 0.00e+00 & 0.00e+00 & -0.00e+00 & 4.67e-07 & 4.43e-07 & 0.170 \\ 
            gpp250-4 & 1.61e-08 & 0.00e+00 & 0.00e+00 & -0.00e+00 & 4.76e-07 & 4.39e-07 & 0.150 \\ 
            gpp500-1 & 4.68e-06 & 0.00e+00 & 0.00e+00 & -0.00e+00 & -2.48e-05 & 2.96e-07 & 0.890 \\ 
            gpp500-2 & 2.10e-07 & 0.00e+00 & 0.00e+00 & -0.00e+00 & -3.84e-07 & 3.25e-07 & 0.800 \\ 
            gpp500-3 & 2.18e-07 & 0.00e+00 & 0.00e+00 & -0.00e+00 & 1.79e-06 & 3.05e-07 & 0.650 \\ 
            gpp500-4 & 8.53e-09 & 0.00e+00 & 0.00e+00 & -0.00e+00 & 2.37e-07 & 2.01e-07 & 0.680 \\ 
              hinf10 & 2.82e-09 & 0.00e+00 & 0.00e+00 & -0.00e+00 & -3.01e-05 & 2.09e-07 & 0.050 \\ 
              hinf11 & 1.68e-09 & 0.00e+00 & 0.00e+00 & -0.00e+00 & -2.88e-05 & 3.51e-07 & 0.050 \\ 
              hinf12 & 3.84e-08 & 0.00e+00 & 0.00e+00 & -0.00e+00 & -2.32e-01 & 9.18e-04 & 0.050 \\ 
              hinf13 & 1.06e-09 & 0.00e+00 & 0.00e+00 & -0.00e+00 & -6.25e-06 & 4.92e-05 & 0.070 \\ 
              hinf14 & 5.06e-08 & 6.05e-15 & 0.00e+00 & -0.00e+00 & -7.15e-08 & 1.83e-07 & 0.080 \\ 
              hinf15 & 1.12e-04 & 0.00e+00 & 0.00e+00 & -0.00e+00 & -2.50e-05 & 1.04e-05 & 0.110 \\ 
               hinf1 & 4.09e-13 & 0.00e+00 & 0.00e+00 & -0.00e+00 & 7.17e-08 & 1.79e-07 & 0.040 \\ 
               hinf2 & 3.59e-10 & 0.00e+00 & 0.00e+00 & -0.00e+00 & 1.03e-07 & 1.63e-07 & 0.050 \\ 
               hinf3 & 4.55e-11 & 0.00e+00 & 0.00e+00 & -0.00e+00 & 1.26e-07 & 1.75e-07 & 0.050 \\ 
               hinf4 & 1.18e-11 & 0.00e+00 & 0.00e+00 & -0.00e+00 & 1.68e-07 & 2.48e-07 & 0.030 \\ 
               hinf5 & 1.65e-03 & 0.00e+00 & 0.00e+00 & -0.00e+00 & 4.23e-06 & 2.84e-07 & 0.050 \\ 
               hinf6 & 9.60e+01 & 0.00e+00 & 7.21e-05 & 0.00e+00 & 4.69e-01 & 3.21e-02 & Failed \\ 
               hinf7 & 3.93e-06 & 0.00e+00 & 0.00e+00 & -0.00e+00 & 1.13e-03 & 1.39e-03 & 0.040 \\ 
               hinf8 & 1.65e-07 & 0.00e+00 & 0.00e+00 & -0.00e+00 & 3.63e-07 & 5.03e-07 & 0.040 \\ 
               hinf9 & 1.03e-06 & 0.00e+00 & 0.00e+00 & -0.00e+00 & 2.28e-07 & 2.17e-07 & 0.050 \\ 
               infd1 & 1.00e+00 & 1.00e+00 & 1.00e+00& 1.00e+00& 1.00e+00 & 1.00e+00 & 0.040 \\ 
      \bottomrule
    \end{tabular}
  }  
\end{center}
\end{table}}}

{\small{\begin{table}[h]
  \begin{center}
    \caption{SDPLIB benchmark \texttt{HDSDP}, Part 2}\label{sdplib-hdsdp-2}
  \resizebox{0.75\textwidth}{!}{%
  \begin{tabular}{cccccccc}
      \toprule
      Instance & Error 1 & Error 2 & Error 3 & Error 4 & Error 5 & Error 6 &
      Time\\
\midrule
               infd2 & 1.00e+00 & 1.00e+00 & 1.00e+00& 1.00e+00& 1.00e+00 & 1.00e+00 & 0.040 \\ 
	             infp1 & 1.00e+00 & 1.00e+00  &1.00e+00 &1.00e+00 &1.00e+00 & 1.00e+00 & 0.110 \\ 
               infp2 & 1.00e+00 & 1.00e+00  &1.00e+00 &1.00e+00 &1.00e+00 & 1.00e+00 & 0.110 \\ 
              maxG11 & 2.23e-14 & 0.00e+00 & 0.00e+00 & -0.00e+00 & 2.45e-07 & 2.45e-07 & 0.600 \\ 
              maxG32 & 1.04e-14 & 0.00e+00 & 0.00e+00 & -0.00e+00 & 2.25e-07 & 2.25e-07 & 4.680 \\ 
              maxG51 & 2.94e-15 & 0.00e+00 & 0.00e+00 & -0.00e+00 & 5.08e-07 & 5.08e-07 & 1.450 \\ 
              maxG55 & 1.58e-15 & 0.00e+00 & 0.00e+00 & -0.00e+00 & 4.63e-07 & 4.63e-07 & 38.210 \\ 
              maxG60 & 7.29e-16 & 0.00e+00 & 0.00e+00 & -0.00e+00 & 4.29e-07 & 4.29e-07 & 87.590 \\ 
              mcp100 & 4.87e-14 & 0.00e+00 & 0.00e+00 & -0.00e+00 & 2.79e-07 & 2.79e-07 & 0.040 \\ 
            mcp124-1 & 8.40e-15 & 0.00e+00 & 0.00e+00 & -0.00e+00 & 3.36e-07 & 3.36e-07 & 0.040 \\ 
            mcp124-2 & 4.76e-15 & 0.00e+00 & 0.00e+00 & -0.00e+00 & 2.80e-07 & 2.80e-07 & 0.050 \\ 
            mcp124-3 & 1.71e-13 & 0.00e+00 & 0.00e+00 & -0.00e+00 & 2.94e-07 & 2.94e-07 & 0.050 \\ 
            mcp124-4 & 3.35e-14 & 0.00e+00 & 0.00e+00 & -0.00e+00 & 3.94e-07 & 3.94e-07 & 0.060 \\ 
            mcp250-1 & 7.78e-15 & 0.00e+00 & 0.00e+00 & -0.00e+00 & 2.01e-07 & 2.01e-07 & 0.090 \\ 
            mcp250-2 & 3.16e-15 & 0.00e+00 & 0.00e+00 & -0.00e+00 & 1.62e-07 & 1.62e-07 & 0.080 \\ 
            mcp250-3 & 1.74e-14 & 0.00e+00 & 0.00e+00 & -0.00e+00 & 3.64e-07 & 3.64e-07 & 0.090 \\ 
            mcp250-4 & 6.43e-15 & 0.00e+00 & 0.00e+00 & -0.00e+00 & 6.59e-07 & 6.59e-07 & 0.110 \\ 
            mcp500-1 & 2.99e-16 & 0.00e+00 & 0.00e+00 & -0.00e+00 & 4.98e-07 & 4.98e-07 & 0.260 \\ 
            mcp500-2 & 1.26e-14 & 0.00e+00 & 0.00e+00 & -0.00e+00 & 2.33e-07 & 2.33e-07 & 0.250 \\ 
            mcp500-3 & 2.79e-14 & 0.00e+00 & 0.00e+00 & -0.00e+00 & 1.73e-07 & 1.73e-07 & 0.300 \\ 
            mcp500-4 & 2.07e-15 & 0.00e+00 & 0.00e+00 & -0.00e+00 & 3.41e-07 & 3.41e-07 & 0.390 \\ 
               qap10 & 2.11e-11 & 0.00e+00 & 0.00e+00 & -0.00e+00 & 1.52e-05 & 2.17e-05 & 0.640 \\ 
                qap5 & 9.90e-11 & 0.00e+00 & 0.00e+00 & -0.00e+00 & 6.02e-08 & 9.37e-08 & 0.040 \\ 
                qap6 & 2.33e-09 & 0.00e+00 & 0.00e+00 & -0.00e+00 & 1.18e-10 & 8.35e-08 & 0.070 \\ 
                qap7 & 2.45e-09 & 0.00e+00 & 0.00e+00 & -0.00e+00 & 1.14e-08 & 5.99e-08 & 0.090 \\ 
                qap8 & 2.77e-10 & 0.00e+00 & 0.00e+00 & -0.00e+00 & -3.83e-08 & 6.13e-08 & 0.210 \\ 
                qap9 & 5.55e-13 & 0.00e+00 & 0.00e+00 & -0.00e+00 & 7.02e-06 & 1.66e-05 & 0.320 \\ 
               qpG11 & 3.83e-14 & 0.00e+00 & 0.00e+00 & -0.00e+00 & 5.15e-07 & 5.15e-07 & 2.060 \\ 
               qpG51 & 1.66e-13 & 0.00e+00 & 0.00e+00 & -0.00e+00 & 3.21e-07 & 3.21e-07 & 11.840 \\ 
                ss30 & 2.91e-11 & 0.00e+00 & 0.00e+00 & -0.00e+00 & 4.09e-07 & 2.85e-07 & 0.560 \\ 
              theta1 & 9.23e-13 & 0.00e+00 & 0.00e+00 & -0.00e+00 & 1.06e-07 & 1.06e-07 & 0.050 \\ 
              theta2 & 7.53e-14 & 0.00e+00 & 0.00e+00 & -0.00e+00 & 4.72e-08 & 4.72e-08 & 0.130 \\ 
              theta3 & 1.19e-15 & 0.00e+00 & 0.00e+00 & -0.00e+00 & 3.84e-08 & 3.84e-08 & 0.440 \\ 
              theta4 & 1.02e-14 & 0.00e+00 & 0.00e+00 & -0.00e+00 & 2.78e-08 & 2.78e-08 & 1.400 \\ 
              theta5 & 8.89e-16 & 0.00e+00 & 0.00e+00 & -0.00e+00 & 6.87e-08 & 6.87e-08 & 2.850 \\ 
              theta6 & 3.26e-15 & 0.00e+00 & 0.00e+00 & -0.00e+00 & 2.32e-08 & 2.32e-08 & 5.990 \\ 
            thetaG11 & 4.76e-14 & 0.00e+00 & 0.00e+00 & -0.00e+00 & 1.29e-07 & 1.29e-07 & 13.480 \\ 
            thetaG51 & 1.90e-10 & 0.00e+00 & 0.00e+00 & -0.00e+00 & 6.59e-08 & 7.17e-08 & 319.050 \\ 
              truss1 & 1.88e-13 & 0.00e+00 & 0.00e+00 & -0.00e+00 & 5.49e-07 & 5.48e-07 & 0.050 \\ 
              truss2 & 1.14e-11 & 0.00e+00 & 5.75e-10 & 0.00e+00 & 3.78e-07 & 3.78e-07 & 0.390 \\ 
              truss3 & 6.70e-13 & 0.00e+00 & 2.74e-10 & 0.00e+00 & 1.35e-07 & 1.32e-07 & 0.090 \\ 
              truss4 & 1.08e-14 & 0.00e+00 & 2.12e-10 & 0.00e+00 & 3.04e-07 & 2.93e-07 & 0.070 \\ 
              truss5 & 5.16e-12 & 0.00e+00 & 0.00e+00 & -0.00e+00 & 8.93e-08 & 8.92e-08 & 0.770 \\ 
              truss6 & 7.31e-09 & 0.00e+00 & 0.00e+00 & -0.00e+00 & 4.76e-07 & 4.75e-07 & 0.700 \\ 
              truss7 & 1.39e-08 & 0.00e+00 & 0.00e+00 & -0.00e+00 & 3.76e-07 & 3.75e-07 & 0.900 \\ 
              truss8 & 6.82e-12 & 0.00e+00 & 1.25e-09 & 0.00e+00 & 1.46e-07 & 1.46e-07 & 1.740 \\ 
      \bottomrule
    \end{tabular}
  }  
\end{center}
\end{table}}}

{\small{\begin{table}[h]
  \begin{center}
    \caption{SDPLIB benchmark \texttt{DSDP5.8}, Part 1}
  \label{sdplib-dsdp-1}
  \resizebox{0.75\textwidth}{!}{%
  \begin{tabular}{cccccccc}
      \toprule
      Instance & Error 1 & Error 2 & Error 3 & Error 4 & Error 5 & Error 6 &
      Time\\
\midrule
                     arch0 & 2.52e-07 & 0.00e+00 & 0.00e+00 & 0.00e+00 & 2.75e-07 & 3.35e-07 & 0.400 \\ 
               arch2 & 1.62e-07 & 0.00e+00 & 0.00e+00 & 0.00e+00 & 3.34e-07 & 3.59e-07 & 0.318 \\ 
               arch4 & 1.38e-07 & 0.00e+00 & 0.00e+00 & 0.00e+00 & 8.39e-08 & 1.07e-07 & 0.375 \\ 
               arch8 & 7.30e-07 & 0.00e+00 & 0.00e+00 & 0.00e+00 & 1.23e-07 & 2.02e-07 & 0.339 \\ 
           control10 & 8.77e-07 & 0.00e+00 & 0.00e+00 & 0.00e+00 & 8.20e-07 & 3.31e-06 & 7.343 \\ 
           control11 & 7.77e-07 & 0.00e+00 & 0.00e+00 & 0.00e+00 & 2.60e-06 & 5.70e-06 & 12.050 \\ 
            control1 & 4.84e-07 & 0.00e+00 & 0.00e+00 & 0.00e+00 & -1.88e-07 & 3.99e-08 & 0.032 \\ 
            control2 & 2.56e-07 & 0.00e+00 & 0.00e+00 & 0.00e+00 & -4.63e-08 & 8.55e-08 & 0.048 \\ 
            control3 & 3.25e-07 & 0.00e+00 & 0.00e+00 & 0.00e+00 & 1.55e-07 & 2.54e-07 & 0.087 \\ 
            control4 & 1.67e-06 & 0.00e+00 & 0.00e+00 & 0.00e+00 & 2.54e-08 & 3.29e-06 & 0.168 \\ 
            control5 & 5.27e-07 & 0.00e+00 & 0.00e+00 & 0.00e+00 & -4.68e-07 & 5.21e-07 & 0.487 \\ 
            control6 & 3.22e-05 & 0.00e+00 & 0.00e+00 & 0.00e+00 & -1.75e-07 & 7.61e-05 & 0.735 \\ 
            control7 & 3.99e-06 & 0.00e+00 & 0.00e+00 & 0.00e+00 & -4.32e-07 & 1.28e-05 & 2.085 \\ 
            control8 & 7.53e-07 & 0.00e+00 & 0.00e+00 & 0.00e+00 & -3.75e-07 & 1.46e-06 & 3.734 \\ 
            control9 & 8.83e-07 & 0.00e+00 & 0.00e+00 & 0.00e+00 & -6.64e-07 & 1.95e-06 & 4.473 \\ 
            equalG11 & 7.89e-10 & 0.00e+00 & 0.00e+00 & 0.00e+00 & 6.50e-08 & 6.56e-08 & 1.941 \\ 
            equalG51 & 9.93e-10 & 0.00e+00 & 0.00e+00 & 0.00e+00 & 9.23e-08 & 9.33e-08 & 2.917 \\ 
              gpp100 & 1.01e-10 & 0.00e+00 & 0.00e+00 & 0.00e+00 & 3.51e-08 & 4.57e-06 & 0.051 \\ 
            gpp124-1 & 1.25e-10 & 0.00e+00 & 0.00e+00 & 0.00e+00 & 1.90e-07 & 5.51e-05 & 0.074 \\ 
            gpp124-2 & 1.38e-05 & 0.00e+00 & 0.00e+00 & 0.00e+00 & 4.53e-07 & 8.37e-01 & Failed \\ 
            gpp124-3 & 1.28e-10 & 0.00e+00 & 0.00e+00 & 0.00e+00 & 8.71e-08 & 1.60e-06 & 0.063 \\ 
            gpp124-4 & 1.28e-10 & 0.00e+00 & 0.00e+00 & 0.00e+00 & 1.06e-07 & 1.35e-06 & 0.066 \\ 
            gpp250-1 & 2.78e-05 & 0.00e+00 & 0.00e+00 & 0.00e+00 & 1.27e-06 & 9.98e+00 & Failed \\ 
            gpp250-2 & 2.50e-10 & 0.00e+00 & 0.00e+00 & 0.00e+00 & 5.21e-08 & 7.41e-06 & 0.139 \\ 
            gpp250-3 & 2.47e-10 & 0.00e+00 & 0.00e+00 & 0.00e+00 & 4.51e-08 & 1.45e-06 & 0.132 \\ 
            gpp250-4 & 2.48e-10 & 0.00e+00 & 0.00e+00 & 0.00e+00 & 5.61e-08 & 5.82e-07 & 0.137 \\ 
            gpp500-1 & 4.90e-10 & 0.00e+00 & 0.00e+00 & 0.00e+00 & 1.57e-06 & 1.11e-04 & 0.435 \\ 
            gpp500-2 & 4.66e-10 & 0.00e+00 & 0.00e+00 & 0.00e+00 & 5.79e-08 & 1.72e-05 & 0.434 \\ 
            gpp500-3 & 5.19e-10 & 0.00e+00 & 0.00e+00 & 0.00e+00 & 1.26e-07 & 2.45e-06 & 0.355 \\ 
            gpp500-4 & 5.22e-10 & 0.00e+00 & 0.00e+00 & 0.00e+00 & 5.39e-08 & 1.27e-06 & 0.381 \\ 
              hinf10 & 1.72e-08 & 0.00e+00 & 0.00e+00 & 0.00e+00 & -3.10e-05 & 5.76e-06 & 0.029 \\ 
              hinf11 & 8.25e-10 & 0.00e+00 & 0.00e+00 & 0.00e+00 & -3.07e-05 & 8.35e-07 & 0.034 \\ 
              hinf12 & 3.84e-08 & 0.00e+00 & 0.00e+00 & 0.00e+00 & -2.32e-01 & 4.91e-05 & 0.044 \\ 
              hinf13 & 3.11e-08 & 0.00e+00 & 0.00e+00 & 0.00e+00 & -3.94e-05 & 2.68e-04 & 0.041 \\ 
              hinf14 & 1.13e-09 & 0.00e+00 & 0.00e+00 & 0.00e+00 & 6.46e-06 & 2.10e-04 & 0.047 \\ 
              hinf15 & 5.30e-09 & 0.00e+00 & 0.00e+00 & 0.00e+00 & -8.83e-05 & 5.37e-04 & 0.051 \\ 
               hinf1 & 1.03e-09 & 0.00e+00 & 0.00e+00 & 0.00e+00 & 1.05e-09 & 6.17e-05 & 0.028 \\ 
               hinf2 & 2.22e-08 & 0.00e+00 & 0.00e+00 & 0.00e+00 & -3.61e-08 & 1.48e-04 & 0.030 \\ 
               hinf3 & 5.81e-10 & 0.00e+00 & 0.00e+00 & 0.00e+00 & 4.29e-10 & 5.87e-06 & 0.026 \\ 
               hinf4 & 1.19e-09 & 0.00e+00 & 0.00e+00 & 0.00e+00 & -1.11e-09 & 5.44e-08 & 0.030 \\ 
               hinf5 & 6.41e-07 & 0.00e+00 & 0.00e+00 & 0.00e+00 & 1.17e-03 & 3.86e-03 & 0.024 \\ 
               hinf6 & 4.01e-07 & 0.00e+00 & 0.00e+00 & 0.00e+00 & 1.60e-02 & 2.74e-02 & Failed \\ 
               hinf7 & 1.61e-05 & 0.00e+00 & 0.00e+00 & 0.00e+00 & 5.22e-05 & 9.44e-03 & 0.030 \\ 
               hinf8 & 5.62e-08 & 0.00e+00 & 0.00e+00 & 0.00e+00 & -1.03e-06 & 1.51e-03 & 0.027 \\ 
               hinf9 & 3.70e-05 & 0.00e+00 & 0.00e+00 & 0.00e+00 & -2.55e-07 & 6.68e-07 & 0.026 \\ 
               infd1 & 3.33e-01 & 0.00e+00 & 0.00e+00 & 0.00e+00 & -1.00e+00 & 1.79e-08 & 0.038\\
      \bottomrule
    \end{tabular}
  }  
\end{center}
\end{table}}}

{\small{\begin{table}[h]
  \begin{center}
    \caption{SDPLIB benchmark \texttt{DSDP5.8}, Part 2}
  \label{sdplib-dsdp-2}
  \resizebox{0.75\textwidth}{!}{%
  \begin{tabular}{cccccccc}
      \toprule
      Instance & Error 1 & Error 2 & Error 3 & Error 4 & Error 5 & Error 6 &
      Time\\
      \midrule
      infd2 & 4.27e-01 & 0.00e+00 & 0.00e+00 & 0.00e+00 & -1.00e+00 & 2.77e-08 & 0.038 \\ 
               infp1 & 5.80e-04 & 3.01e-01 & 0.00e+00 & 0.00e+00 & -1.00e+00 & 7.01e-10 & 0.035 \\ 
               infp2 & 5.43e-05 & 2.96e-01 & 0.00e+00 & 0.00e+00 & -1.00e+00 & 3.11e-09 & 0.031 \\ 
              maxG11 & 1.43e-09 & 0.00e+00 & 0.00e+00 & 0.00e+00 & 4.83e-08 & 4.88e-08 & 0.462 \\ 
              maxG32 & 2.34e-09 & 0.00e+00 & 0.00e+00 & 0.00e+00 & 7.10e-08 & 7.14e-08 & 3.659 \\ 
              maxG51 & 1.60e-09 & 0.00e+00 & 0.00e+00 & 0.00e+00 & 1.16e-07 & 1.21e-07 & 2.519 \\ 
              maxG55 & 3.57e-09 & 0.00e+00 & 0.00e+00 & 0.00e+00 & 5.86e-07 & 5.90e-07 & 273.600 \\ 
              maxG60 & 4.22e-09 & 0.00e+00 & 0.00e+00 & 0.00e+00 & 3.60e-07 & 3.62e-07 & 535.200 \\ 
              mcp100 & 5.06e-10 & 0.00e+00 & 0.00e+00 & 0.00e+00 & 6.03e-08 & 6.41e-08 & 0.015 \\ 
            mcp124-1 & 5.62e-10 & 0.00e+00 & 0.00e+00 & 0.00e+00 & 1.39e-07 & 2.16e-07 & 0.016 \\ 
            mcp124-2 & 5.63e-10 & 0.00e+00 & 0.00e+00 & 0.00e+00 & 9.95e-08 & 1.04e-07 & 0.018 \\ 
            mcp124-3 & 5.63e-10 & 0.00e+00 & 0.00e+00 & 0.00e+00 & 7.73e-08 & 8.15e-08 & 0.024 \\ 
            mcp124-4 & 1.12e-11 & 0.00e+00 & 0.00e+00 & 0.00e+00 & 1.18e-07 & 1.23e-07 & 0.054 \\ 
            mcp250-1 & 7.98e-10 & 0.00e+00 & 0.00e+00 & 0.00e+00 & 9.12e-08 & 9.94e-08 & 0.084 \\ 
            mcp250-2 & 7.99e-10 & 0.00e+00 & 0.00e+00 & 0.00e+00 & 1.05e-07 & 1.17e-07 & 0.090 \\ 
            mcp250-3 & 7.98e-10 & 0.00e+00 & 0.00e+00 & 0.00e+00 & 9.31e-08 & 9.78e-08 & 0.123 \\ 
            mcp250-4 & 7.98e-10 & 0.00e+00 & 0.00e+00 & 0.00e+00 & 4.93e-08 & 5.22e-08 & 0.160 \\ 
            mcp500-1 & 1.13e-09 & 0.00e+00 & 0.00e+00 & 0.00e+00 & 1.06e-07 & 1.53e-07 & 0.217 \\ 
            mcp500-2 & 1.13e-09 & 0.00e+00 & 0.00e+00 & 0.00e+00 & 7.73e-08 & 8.12e-08 & 0.320 \\ 
            mcp500-3 & 1.13e-09 & 0.00e+00 & 0.00e+00 & 0.00e+00 & 1.49e-07 & 1.53e-07 & 0.496 \\ 
            mcp500-4 & 1.13e-09 & 0.00e+00 & 0.00e+00 & 0.00e+00 & 5.69e-08 & 5.93e-08 & 0.862 \\ 
               qap10 & 1.13e-11 & 0.00e+00 & 0.00e+00 & 0.00e+00 & 4.87e-07 & 1.06e-06 & 0.626 \\ 
                qap5 & 4.70e-10 & 0.00e+00 & 0.00e+00 & 0.00e+00 & 1.61e-07 & 8.36e-06 & 0.049 \\ 
                qap6 & 6.49e-12 & 0.00e+00 & 0.00e+00 & 0.00e+00 & -4.47e-08 & 1.91e-07 & 0.065 \\ 
                qap7 & 4.61e-12 & 0.00e+00 & 0.00e+00 & 0.00e+00 & -2.55e-08 & 1.68e-07 & 0.113 \\ 
                qap8 & 9.48e-12 & 0.00e+00 & 0.00e+00 & 0.00e+00 & -8.16e-08 & 1.25e-07 & 0.207 \\ 
                qap9 & 6.48e-12 & 0.00e+00 & 0.00e+00 & 0.00e+00 & -2.13e-08 & 7.09e-08 & 0.364 \\ 
               qpG11 & 1.44e-09 & 0.00e+00 & 0.00e+00 & 0.00e+00 & 1.04e-07 & 1.04e-07 & 1.446 \\ 
               qpG51 & 1.61e-09 & 0.00e+00 & 0.00e+00 & 0.00e+00 & 2.47e-07 & 2.47e-07 & 16.050 \\ 
                ss30 & 4.68e-07 & 0.00e+00 & 0.00e+00 & 0.00e+00 & 1.18e-07 & 1.43e-07 & 0.889 \\ 
              theta1 & 4.75e-11 & 0.00e+00 & 0.00e+00 & 0.00e+00 & 4.54e-08 & 5.24e-08 & 0.045 \\ 
              theta2 & 5.05e-11 & 0.00e+00 & 0.00e+00 & 0.00e+00 & 4.27e-09 & 5.10e-09 & 0.105 \\ 
              theta3 & 7.55e-11 & 0.00e+00 & 0.00e+00 & 0.00e+00 & 1.78e-08 & 2.11e-08 & 0.310 \\ 
              theta4 & 1.00e-10 & 0.00e+00 & 0.00e+00 & 0.00e+00 & 5.30e-09 & 6.37e-09 & 0.963 \\ 
              theta5 & 1.25e-10 & 0.00e+00 & 0.00e+00 & 0.00e+00 & 3.13e-08 & 3.73e-08 & 2.190 \\ 
              theta6 & 1.51e-10 & 0.00e+00 & 0.00e+00 & 0.00e+00 & 4.59e-08 & 5.45e-08 & 4.603 \\ 
            thetaG11 & 6.22e-09 & 0.00e+00 & 0.00e+00 & 0.00e+00 & 6.31e-08 & 6.35e-08 & 10.860 \\ 
            thetaG51 & 1.52e-08 & 0.00e+00 & 0.00e+00 & 0.00e+00 & 3.56e-07 & 4.20e-07 & 96.130 \\ 
              truss1 & 6.52e-12 & 0.00e+00 & 0.00e+00 & 0.00e+00 & 5.39e-09 & 6.94e-09 & 0.026 \\ 
              truss2 & 2.61e-11 & 0.00e+00 & 0.00e+00 & 0.00e+00 & 2.03e-08 & 2.14e-08 & 0.050 \\ 
              truss3 & 7.31e-10 & 0.00e+00 & 0.00e+00 & 0.00e+00 & 2.82e-09 & 3.01e-09 & 0.035 \\ 
              truss4 & 1.77e-11 & 0.00e+00 & 0.00e+00 & 0.00e+00 & 9.49e-10 & 1.69e-09 & 0.026 \\ 
              truss5 & 3.84e-11 & 0.00e+00 & 0.00e+00 & 0.00e+00 & 1.34e-08 & 3.80e-08 & 0.147 \\ 
              truss6 & 1.71e-07 & 0.00e+00 & 0.00e+00 & 0.00e+00 & 1.42e-07 & 2.76e-07 & 0.107 \\ 
              truss7 & 2.68e-06 & 0.00e+00 & 0.00e+00 & 0.00e+00 & 1.58e-09 & 2.01e-08 & 0.070 \\ 
              truss8 & 4.67e-11 & 0.00e+00 & 0.00e+00 & 0.00e+00 & 2.50e-08 & 1.19e-07 & 0.569 \\ 
      \bottomrule
    \end{tabular}
  }  
\end{center}  
\end{table}}}

{\small{\begin{table}[h]
  \begin{center}
    \caption{SDPLIB benchmark \texttt{COPT}, Part 1}
  \label{sdplib-copt-1}
  \resizebox{0.75\textwidth}{!}{%
  \begin{tabular}{cccccccc}
      \toprule
      Instance & Error 1 & Error 2 & Error 3 & Error 4 & Error 5 & Error 6 &
      Time\\
\midrule
                arch0 & 4.48e-07 & 0.00e+00 & 0.00e+00 & 0.00e+00 & -3.52e-09 & 8.67e-07 & 0.700 \\ 
               arch2 & 4.51e-07 & 0.00e+00 & 3.56e-07 & 0.00e+00 & -3.11e-09 & 6.87e-07 & 0.720 \\ 
               arch4 & 6.58e-08 & 0.00e+00 & 0.00e+00 & 0.00e+00 & -5.78e-10 & 1.40e-07 & 0.760 \\ 
               arch8 & 1.75e-08 & 0.00e+00 & 0.00e+00 & 0.00e+00 & -2.48e-10 & 8.99e-08 & 0.880 \\ 
           control10 & 5.36e-09 & 0.00e+00 & 6.11e-11 & 0.00e+00 & -3.91e-07 & 6.54e-05 & 1.800 \\ 
           control11 & 5.18e-09 & 0.00e+00 & 5.36e-11 & 0.00e+00 & -4.07e-07 & 7.46e-05 & 2.640 \\ 
            control1 & 5.75e-10 & 0.00e+00 & 2.63e-10 & 0.00e+00 & -2.25e-09 & 3.03e-08 & 0.030 \\ 
            control2 & 2.67e-10 & 0.00e+00 & 2.92e-10 & 0.00e+00 & -2.71e-09 & 7.20e-08 & 0.040 \\ 
            control3 & 1.51e-09 & 0.00e+00 & 4.44e-12 & 0.00e+00 & -2.92e-08 & 1.31e-06 & 0.050 \\ 
            control4 & 3.88e-09 & 0.00e+00 & 6.33e-10 & 0.00e+00 & -7.48e-08 & 4.66e-06 & 0.080 \\ 
            control5 & 1.71e-09 & 0.00e+00 & 7.87e-12 & 0.00e+00 & -2.65e-08 & 2.13e-06 & 0.170 \\ 
            control6 & 5.64e-09 & 0.00e+00 & 1.90e-11 & 0.00e+00 & -1.87e-07 & 1.84e-05 & 0.320 \\ 
            control7 & 9.12e-10 & 0.00e+00 & 1.78e-11 & 0.00e+00 & -4.96e-08 & 5.51e-06 & 0.390 \\ 
            control8 & 1.14e-09 & 0.00e+00 & 1.92e-11 & 0.00e+00 & -5.65e-08 & 7.30e-06 & 0.670 \\ 
            control9 & 3.49e-10 & 0.00e+00 & 2.12e-11 & 0.00e+00 & -2.27e-08 & 3.29e-06 & 0.940 \\ 
            equalG11 & 4.17e-09 & 0.00e+00 & 0.00e+00 & 0.00e+00 & 2.34e-09 & 1.23e-06 & 8.820 \\ 
            equalG51 & 2.12e-08 & 0.00e+00 & 0.00e+00 & 0.00e+00 & -4.58e-09 & 1.21e-06 & 18.360 \\ 
              gpp100 & 2.97e-07 & 0.00e+00 & 0.00e+00 & 0.00e+00 & 2.82e-08 & 8.89e-07 & 0.190 \\ 
            gpp124-1 & 2.20e-08 & 0.00e+00 & 0.00e+00 & 0.00e+00 & 2.88e-09 & 7.19e-07 & 0.330 \\ 
            gpp124-2 & 2.09e-08 & 0.00e+00 & 7.68e-09 & 0.00e+00 & 5.65e-09 & 3.77e-07 & 0.300 \\ 
            gpp124-3 & 2.30e-08 & 0.00e+00 & 9.30e-09 & 0.00e+00 & 7.20e-09 & 1.69e-07 & 0.310 \\ 
            gpp124-4 & 3.17e-08 & 0.00e+00 & 5.91e-09 & 0.00e+00 & 3.89e-09 & 2.15e-07 & 0.290 \\ 
            gpp250-1 & 1.83e-07 & 0.00e+00 & 0.00e+00 & 0.00e+00 & 1.12e-08 & 6.77e-07 & 1.650 \\ 
            gpp250-2 & 4.76e-07 & 0.00e+00 & 0.00e+00 & 0.00e+00 & 3.87e-08 & 1.10e-06 & 1.210 \\ 
            gpp250-3 & 1.09e-07 & 0.00e+00 & 0.00e+00 & 0.00e+00 & 9.83e-09 & 2.93e-07 & 1.410 \\ 
            gpp250-4 & 3.34e-08 & 0.00e+00 & 7.83e-09 & 0.00e+00 & 2.78e-09 & 1.02e-07 & 1.520 \\ 
            gpp500-1 & 5.44e-07 & 0.00e+00 & 0.00e+00 & 0.00e+00 & 1.88e-08 & 1.16e-06 & 5.520 \\ 
            gpp500-2 & 8.13e-08 & 0.00e+00 & 0.00e+00 & 0.00e+00 & 7.80e-09 & 3.38e-07 & 5.430 \\ 
            gpp500-3 & 1.11e-07 & 0.00e+00 & 0.00e+00 & 0.00e+00 & 1.05e-08 & 1.91e-07 & 5.530 \\ 
            gpp500-4 & 8.68e-09 & 0.00e+00 & 0.00e+00 & 0.00e+00 & 2.33e-09 & 4.27e-08 & 5.400 \\ 
              hinf10 & 6.72e-09 & 0.00e+00 & 6.16e-09 & 0.00e+00 & -3.79e-08 & 5.88e-07 & 0.040 \\ 
              hinf11 & 3.33e-08 & 0.00e+00 & 0.00e+00 & 0.00e+00 & -4.88e-08 & 1.22e-06 & 0.050 \\ 
              hinf12 & 2.32e-16 & 0.00e+00 & 0.00e+00 & 0.00e+00 & -3.66e-13 & 4.29e-12 & 0.070 \\ 
              hinf13 & 1.50e-06 & 0.00e+00 & 0.00e+00 & 0.00e+00 & -1.49e-04 & 3.44e-03 & 0.050 \\ 
              hinf14 & 1.84e-07 & 0.00e+00 & 0.00e+00 & 0.00e+00 & -1.30e-06 & 4.22e-05 & 0.060 \\ 
              hinf15 & 3.01e-05 & 0.00e+00 & 0.00e+00 & 0.00e+00 & -8.02e-05 & 2.90e-03 & 0.050 \\ 
               hinf1 & 1.58e-08 & 0.00e+00 & 0.00e+00 & 0.00e+00 & -1.54e-06 & 1.70e-05 & 0.030 \\ 
               hinf2 & 4.25e-07 & 0.00e+00 & 0.00e+00 & 0.00e+00 & -1.07e-06 & 1.65e-05 & 0.030 \\ 
               hinf3 & 3.17e-07 & 0.00e+00 & 0.00e+00 & 0.00e+00 & -1.71e-06 & 2.56e-05 & 0.030 \\ 
               hinf4 & 1.39e-07 & 0.00e+00 & 4.09e-13 & 0.00e+00 & -1.97e-07 & 3.06e-06 & 0.030 \\ 
               hinf5 & 1.05e-07 & 0.00e+00 & 0.00e+00 & 0.00e+00 & -4.01e-06 & 6.13e-05 & 0.030 \\ 
               hinf6 & 8.33e-06 & 0.00e+00 & 0.00e+00 & 0.00e+00 & -6.60e-07 & 9.27e-06 & 0.040 \\ 
               hinf7 & 2.71e-05 & 0.00e+00 & 8.00e-11 & 0.00e+00 & -2.25e-07 & 4.67e-06 & 0.040 \\ 
               hinf8 & 5.06e-08 & 0.00e+00 & 0.00e+00 & 0.00e+00 & -2.04e-06 & 3.01e-05 & 0.030 \\ 
               hinf9 & 3.12e-05 & 0.00e+00 & 0.00e+00 & 0.00e+00 & -3.25e-06 & 2.13e-04 & 0.040 \\ 
               infd1 & 1.87e+00 & 0.00e+00 & 0.00e+00 & 0.00e+00 & -6.97e-01 & 9.10e+00 & 0.040 \\ 
      \bottomrule
    \end{tabular}
  }  
\end{center}
\end{table}}}

{\small{\begin{table}[h]
  \begin{center}
    \caption{SDPLIB benchmark \texttt{COPT}, Part 2}
    \label{sdplib-copt-2}
  \resizebox{0.75\textwidth}{!}{%
  \begin{tabular}{cccccccc}
      \toprule
      Instance & Error 1 & Error 2 & Error 3 & Error 4 & Error 5 & Error 6 &
      Time\\
      \midrule
               infd2 & 1.95e+00 & 0.00e+00 & 0.00e+00 & 0.00e+00 & -9.77e-01 & 1.15e+01 & 0.030 \\ 
               infp1 & 7.85e-01 & 0.00e+00 & 0.00e+00 & 0.00e+00 & -1.58e-01 & 2.53e+01 & 0.030 \\ 
               infp2 & 1.52e+00 & 0.00e+00 & 0.00e+00 & 0.00e+00 & -1.88e-01 & 2.44e+01 & 0.030 \\ 
              maxG11 & 3.45e-12 & 0.00e+00 & 0.00e+00 & 0.00e+00 & -1.37e-09 & 1.09e-07 & 7.150 \\ 
              maxG32 & 1.66e-11 & 0.00e+00 & 0.00e+00 & 0.00e+00 & -2.42e-10 & 7.31e-08 & 68.320 \\ 
              maxG51 & 2.84e-10 & 0.00e+00 & 0.00e+00 & 0.00e+00 & -4.30e-09 & 2.98e-09 & 14.400 \\ 
              maxG55 & 1.07e-10 & 0.00e+00 & 0.00e+00 & 0.00e+00 & -1.32e-09 & 1.83e-09 & 1096.020 \\ 
              maxG60 & 5.47e-11 & 0.00e+00 & 0.00e+00 & 0.00e+00 & -1.14e-09 & 1.81e-09 & 2926.110 \\ 
              mcp100 & 5.89e-12 & 0.00e+00 & 0.00e+00 & 0.00e+00 & -1.72e-09 & 2.43e-09 & 0.110 \\ 
            mcp124-1 & 6.60e-12 & 0.00e+00 & 0.00e+00 & 0.00e+00 & -5.65e-10 & 1.44e-09 & 0.170 \\ 
            mcp124-2 & 8.59e-12 & 0.00e+00 & 0.00e+00 & 0.00e+00 & -6.00e-10 & 8.80e-10 & 0.170 \\ 
            mcp124-3 & 1.02e-11 & 0.00e+00 & 0.00e+00 & 0.00e+00 & -4.61e-09 & 4.16e-09 & 0.160 \\ 
            mcp124-4 & 2.02e-11 & 0.00e+00 & 0.00e+00 & 0.00e+00 & -7.56e-10 & 4.17e-10 & 0.170 \\ 
            mcp250-1 & 3.10e-12 & 0.00e+00 & 0.00e+00 & 0.00e+00 & -4.52e-09 & 1.09e-08 & 0.700 \\ 
            mcp250-2 & 5.81e-12 & 0.00e+00 & 0.00e+00 & 0.00e+00 & -1.26e-09 & 1.96e-09 & 0.720 \\ 
            mcp250-3 & 2.52e-10 & 0.00e+00 & 0.00e+00 & 0.00e+00 & -4.78e-09 & 4.37e-09 & 0.650 \\ 
            mcp250-4 & 1.20e-09 & 0.00e+00 & 0.00e+00 & 0.00e+00 & -9.63e-10 & 5.72e-10 & 0.710 \\ 
            mcp500-1 & 4.38e-12 & 0.00e+00 & 0.00e+00 & 0.00e+00 & -3.84e-09 & 9.63e-09 & 2.780 \\ 
            mcp500-2 & 1.31e-09 & 0.00e+00 & 0.00e+00 & 0.00e+00 & -1.03e-09 & 1.61e-09 & 2.820 \\ 
            mcp500-3 & 2.44e-11 & 0.00e+00 & 0.00e+00 & 0.00e+00 & -1.88e-09 & 1.86e-09 & 2.590 \\ 
            mcp500-4 & 1.75e-11 & 0.00e+00 & 0.00e+00 & 0.00e+00 & -8.25e-10 & 4.85e-10 & 2.860 \\ 
               qap10 & 8.86e-08 & 0.00e+00 & 9.13e-13 & 0.00e+00 & -3.19e-08 & 3.42e-06 & 0.610 \\ 
                qap5 & 7.91e-08 & 0.00e+00 & 0.00e+00 & 0.00e+00 & 1.89e-09 & 1.10e-07 & 0.030 \\ 
                qap6 & 4.72e-08 & 0.00e+00 & 8.86e-13 & 0.00e+00 & -1.03e-07 & 3.72e-06 & 0.070 \\ 
                qap7 & 4.17e-08 & 0.00e+00 & 5.04e-13 & 0.00e+00 & -6.60e-08 & 3.35e-06 & 0.120 \\ 
                qap8 & 1.12e-07 & 0.00e+00 & 6.18e-13 & 0.00e+00 & -8.25e-08 & 5.96e-06 & 0.220 \\ 
                qap9 & 1.02e-07 & 0.00e+00 & 5.11e-13 & 0.00e+00 & -2.88e-08 & 2.60e-06 & 0.360 \\ 
               qpG11 & 3.53e-06 & 0.00e+00 & 0.00e+00 & 0.00e+00 & -1.23e-10 & 2.90e-07 & 34.900 \\ 
               qpG51 & 8.21e-06 & 0.00e+00 & 0.00e+00 & 0.00e+00 & -1.83e-10 & 5.41e-07 & 85.440 \\ 
                ss30 & 2.81e-07 & 0.00e+00 & 3.74e-07 & 0.00e+00 & -3.06e-09 & 4.40e-07 & 2.190 \\ 
              theta1 & 2.83e-08 & 0.00e+00 & 0.00e+00 & 0.00e+00 & -1.60e-09 & 4.22e-08 & 0.050 \\ 
              theta2 & 7.40e-09 & 0.00e+00 & 0.00e+00 & 0.00e+00 & -4.11e-10 & 1.70e-08 & 0.150 \\ 
              theta3 & 2.88e-08 & 0.00e+00 & 0.00e+00 & 0.00e+00 & -9.03e-10 & 5.20e-08 & 0.380 \\ 
              theta4 & 1.01e-08 & 0.00e+00 & 0.00e+00 & 0.00e+00 & -3.56e-10 & 1.99e-08 & 1.130 \\ 
              theta5 & 7.99e-09 & 0.00e+00 & 0.00e+00 & 0.00e+00 & -2.74e-10 & 1.69e-08 & 1.700 \\ 
              theta6 & 7.71e-09 & 0.00e+00 & 0.00e+00 & 0.00e+00 & -2.78e-10 & 2.18e-08 & 2.890 \\ 
            thetaG11 & 1.90e-07 & 0.00e+00 & 0.00e+00 & 0.00e+00 & -4.65e-09 & 1.52e-07 & 7.750 \\ 
            thetaG51 & 1.08e-07 & 0.00e+00 & 0.00e+00 & 0.00e+00 & -1.98e-09 & 6.69e-08 & 35.380 \\ 
              truss1 & 1.90e-08 & 0.00e+00 & 0.00e+00 & 0.00e+00 & -3.41e-09 & 4.60e-08 & 0.020 \\ 
              truss2 & 7.82e-08 & 0.00e+00 & 0.00e+00 & 0.00e+00 & -2.46e-09 & 3.64e-07 & 0.040 \\ 
              truss3 & 2.05e-08 & 0.00e+00 & 0.00e+00 & 0.00e+00 & -1.02e-09 & 4.66e-08 & 0.030 \\ 
              truss4 & 1.93e-08 & 0.00e+00 & 0.00e+00 & 0.00e+00 & -2.32e-09 & 4.46e-08 & 0.030 \\ 
              truss5 & 4.30e-08 & 0.00e+00 & 0.00e+00 & 0.00e+00 & -4.60e-10 & 1.68e-07 & 0.070 \\ 
              truss6 & 1.24e-07 & 0.00e+00 & 0.00e+00 & 0.00e+00 & -3.37e-09 & 1.74e-06 & 0.060 \\ 
              truss7 & 7.24e-08 & 0.00e+00 & 0.00e+00 & 0.00e+00 & -3.52e-09 & 1.23e-06 & 0.050 \\ 
              truss8 & 4.21e-07 & 0.00e+00 & 0.00e+00 & 0.00e+00 & -2.13e-09 & 1.50e-06 & 0.220 \\ 
      \bottomrule
    \end{tabular}
  }  
\end{center}  
\end{table}}}




